A Classification Benchmark for Artificial Intelligence Detection of Laryngeal Cancer from Patient Voice

Cases of laryngeal cancer are predicted to rise significantly in the coming years. Current diagnostic pathways are inefficient, putting undue stress on both patients and the medical system. Artificial intelligence offers a promising solution by enabling non-invasive detection of laryngeal cancer from patient voice, which could help prioritise referrals more effectively. A major barrier in this field is the lack of reproducible methods. Our work addresses this challenge by introducing a benchmark suite comprising 36 models trained and evaluated on open-source datasets. These models classify patients with benign and malignant voice pathologies. All models are accessible in a public repository, providing a foundation for future research. We evaluate three algorithms and three audio feature sets, including both audio-only inputs and multimodal inputs incorporating demographic and symptom data. Our best model achieves a balanced accuracy of 83.7%, sensitivity of 84.0%, specificity of 83.3%, and AUROC of 91.8%.

==> SymptomsResultsTable.tex <==
\begin{table*}[ht]
\vspace*{-2cm}
\fontsize{8}{10}\selectfont
\centering
\begin{tabular}{x{1.5cm}|x{2cm}|c|ccc}

\multirow[c]{2}{*}{Classifier} & \multirow[c]{2}{*}{Inputs} & \multirow[c]{2}{*}{Metric} & \multicolumn{3}{c}{FEMH (holdout test dataset)}  \\

&  &  & FeatureStates & OpenSmile & MFCC  \\
\hline

\multirow[c]{8}{*}{\makecell[c]{SVM}} & \multirow[c]{4}{*}{\makecell[c]{Voice + \\Demographics + \\Symptoms}} & Balanced Accuracy & \makecell[t]{0.766 \\ (0.671, 0.848)} & \makecell[t]{\textbf{0.807} \\ (0.720, 0.872)} & \makecell[t]{0.793 \\ (0.707, 0.862)} \\
& & Sensitivity & \makecell[t]{0.720 \\ (0.526, 0.880)} & \makecell[t]{\textbf{0.840} \\ (0.678, 0.962)} & \makecell[t]{\textbf{0.840} \\ (0.667, 0.966)}  \\
& & Specificity & \makecell[t]{\textbf{0.811} \\ (0.780, 0.841)} & \makecell[t]{0.775 \\ (0.741, 0.807)} & \makecell[t]{0.746 \\ (0.714, 0.780)}  \\
& & AUROC & \makecell[t]{0.863 \\ (0.799, 0.918)} & \makecell[t]{\textbf{0.893} \\ (0.835, 0.937)} & \makecell[t]{0.848 \\ (0.796, 0.892)}  \\
\cline{2-6} 
&\multirow[c]{4}{*}{\makecell[c]{Voice + \\Symptoms}} & Balanced Accuracy & \makecell[t]{0.813 \\ (0.720, 0.886)} & \makecell[t]{\textbf{0.814} \\ (0.725, 0.891)} & \makecell[t]{0.697 \\ (0.597, 0.795)}  \\
& & Sensitivity & \makecell[t]{\textbf{0.800} \\ (0.609, 0.950)} & \makecell[t]{\textbf{0.800} \\ (0.619, 0.950)} & \makecell[t]{0.640 \\ (0.438, 0.826)}  \\
& & Specificity & \makecell[t]{0.827 \\ (0.796, 0.857)} & \makecell[t]{\textbf{0.828} \\ (0.799, 0.856)} & \makecell[t]{0.754 \\ (0.722, 0.788)}  \\
& & AUROC & \makecell[t]{0.859 \\ (0.785, 0.918)} & \makecell[t]{\textbf{0.866} \\ (0.798, 0.918)} & \makecell[t]{0.804 \\ (0.723, 0.879)}  \\


\hline
\hline


\multirow[c]{8}{*}{\makecell[c]{MLP}} & \multirow[c]{4}{*}{\makecell[c]{Voice + \\Demographics + \\Symptoms}} & Balanced Accuracy & \makecell[t]{0.695 \\ (0.596, 0.800)} & \makecell[t]{\textbf{0.776} \\ (0.673, 0.859)} & \makecell[t]{0.779 \\ (0.676, 0.872)}  \\
& & Sensitivity & \makecell[t]{0.440 \\ (0.241, 0.647)} & \makecell[t]{\textbf{0.720} \\ (0.516, 0.885)} & \makecell[t]{0.680 \\ (0.483, 0.867)}  \\
& & Specificity & \makecell[t]{\textbf{0.950} \\ (0.931, 0.967)} & \makecell[t]{0.831 \\ (0.801, 0.859)} & \makecell[t]{0.877 \\ (0.852, 0.903)}  \\
& & AUROC & \makecell[t]{0.865 \\ (0.787, 0.933)} & \makecell[t]{\textbf{0.892} \\ (0.839, 0.937)} & \makecell[t]{0.883 \\ (0.828, 0.936)}  \\
\cline{2-6} 
&\multirow[c]{4}{*}{\makecell[c]{Voice + \\Symptoms}} & Balanced Accuracy & \makecell[t]{0.742 \\ (0.641, 0.838)} & \makecell[t]{\textbf{0.792} \\ (0.701, 0.873)} & \makecell[t]{0.786 \\ (0.698, 0.857)}  \\
& & Sensitivity & \makecell[t]{0.640 \\ (0.440, 0.826)} & \makecell[t]{0.760 \\ (0.571, 0.920)} & \makecell[t]{\textbf{0.800} \\ (0.619, 0.946)}  \\
& & Specificity & \makecell[t]{\textbf{0.844} \\ (0.817, 0.873)} & \makecell[t]{0.824 \\ (0.791, 0.851)} & \makecell[t]{0.772 \\ (0.739, 0.803)}  \\
& & AUROC & \makecell[t]{0.839 \\ (0.764, 0.903)} & \makecell[t]{\textbf{0.889} \\ (0.834, 0.936)} & \makecell[t]{0.865 \\ (0.802, 0.919)}  \\

\hline
\hline
\multirow[c]{8}{*}{\makecell[c]{Logistic \\Regression}} & \multirow[c]{4}{*}{\makecell[c]{Voice + \\Demographics + \\Symptoms}} & Balanced Accuracy & \makecell[t]{0.798 \\ (0.711, 0.871)} & \makecell[t]{\textbf{0.837} \\ (0.752, 0.901)} & \makecell[t]{0.827 \\ (0.754, 0.887)}  \\
& & Sensitivity & \makecell[t]{0.800 \\ (0.633, 0.947)} & \makecell[t]{0.840 \\ (0.680, 0.966)} & \makecell[t]{\textbf{0.880} \\ (0.737, 1.000)}  \\
& & Specificity & \makecell[t]{0.797 \\ (0.765, 0.826)} & \makecell[t]{\textbf{0.833} \\ (0.802, 0.862)} & \makecell[t]{0.773 \\ (0.741, 0.806)}  \\
& & AUROC & \makecell[t]{0.896 \\ (0.844, 0.941)} & \makecell[t]{\textbf{0.918} \\ (0.871, 0.954)} & \makecell[t]{0.910 \\ (0.863, 0.948)}  \\
\cline{2-6} 
&\multirow[c]{4}{*}{\makecell[c]{Voice + \\Symptoms}} & Balanced Accuracy & \makecell[t]{\textbf{0.807} \\ (0.723, 0.874)} & \makecell[t]{0.786 \\ (0.695, 0.869)} & \makecell[t]{0.806 \\ (0.719, 0.874)}  \\
& & Sensitivity & \makecell[t]{\textbf{0.840} \\ (0.677, 0.966)} & \makecell[t]{0.760 \\ (0.579, 0.923)} & \makecell[t]{\textbf{0.840} \\ (0.667, 0.966)}  \\
& & Specificity & \makecell[t]{0.773 \\ (0.739, 0.806)} & \makecell[t]{\textbf{0.813} \\ (0.782, 0.842)} & \makecell[t]{0.772 \\ (0.738, 0.806)}  \\
& & AUROC & \makecell[t]{0.868 \\ (0.797, 0.927)} & \makecell[t]{\textbf{0.879} \\ (0.831, 0.922)} & \makecell[t]{0.878 \\ (0.821, 0.925)}  \\



\end{tabular}
\caption{Classification results for the three acoustic features combined with the demographics and symptoms. These models could only be evaluated on a holdout test set from the FEMH dataset, as the external test set (SVD) does not include the required symptom data. Bold values are the highest for that metric and test set. SVM - support vector machine, MLP - multi-layered perceptron.}
\label{tab:ClassificationResults-Symptoms}
\end{table*}

==> VoiceDemographicsResultsTable.tex <==
\begin{table*}[t]
% \vspace*{-2cm}
\fontsize{8}{8}\selectfont
% \begin{adjustwidth}{-1.2cm}{-1.2cm}
\centering
% \setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.75}
\begin{tabular}{x{1.5cm}|x{1.85cm}|x{1.5cm}|ccc|ccc}

 &  &  & \multicolumn{3}{c|}{FEMH (holdout test set)} & \multicolumn{3}{c}{SVD (external test set)} \\
 \hline
 &  &  & FeatureStates & OpenSmile & MFCC & FeatureStates & OpenSmile & MFCC \\
\hline
\multirow[c]{8}{*}{SVM} & \multirow[c]{4}{*}{Voice} & Balanced Accuracy & \makecell[t]{\textbf{0.691} \\ (0.593, 0.784)} & \makecell[t]{0.680 \\ (0.580, 0.772)} & \makecell[t]{0.631 \\ (0.531, 0.731)} & \makecell[t]{\textbf{0.628} \\ (0.557, 0.696)} & \makecell[t]{0.582 \\ (0.497, 0.662)} & \makecell[t]{0.532 \\ (0.462, 0.613)} \\
 &  & Sensitivity & \makecell[t]{\textbf{0.680} \\ (0.480, 0.857)} & \makecell[t]{0.640 \\ (0.440, 0.818)} & \makecell[t]{0.400 \\ (0.206, 0.609)} & \makecell[t]{\textbf{0.763} \\ (0.621, 0.900)} & \makecell[t]{0.500 \\ (0.341, 0.667)} & \makecell[t]{0.289 \\ (0.154, 0.455)} \\
 &  & Specificity & \makecell[t]{0.702 \\ (0.665, 0.736)} & \makecell[t]{0.720 \\ (0.686, 0.754)} & \makecell[t]{\textbf{0.861} \\ (0.835, 0.887)} & \makecell[t]{0.493 \\ (0.466, 0.521)} & \makecell[t]{0.663 \\ (0.637, 0.690)} & \makecell[t]{\textbf{0.775} \\ (0.752, 0.799)} \\
 &  & AUROC & \makecell[t]{\textbf{0.760} \\ (0.665, 0.845)} & \makecell[t]{0.742 \\ (0.676, 0.805)} & \makecell[t]{0.701 \\ (0.594, 0.807)} & \makecell[t]{\textbf{0.649} \\ (0.562, 0.735)} & \makecell[t]{0.615 \\ (0.522, 0.711)} & \makecell[t]{0.592 \\ (0.503, 0.679)} \\
\cline{2-9}
 & \multirow[c]{4}{*}{\makecell[c]{Voice + \\ Demographics}} & Balanced Accuracy & \makecell[t]{0.700 \\ (0.594, 0.789)} & \makecell[t]{\textbf{0.752} \\ (0.656, 0.837)} & \makecell[t]{0.701 \\ (0.599, 0.803)} & \makecell[t]{0.609 \\ (0.529, 0.691)} & \makecell[t]{0.646 \\ (0.566, 0.730)} & \makecell[t]{\textbf{0.681} \\ (0.599, 0.759)} \\
 &  & Sensitivity & \makecell[t]{0.640 \\ (0.429, 0.818)} & \makecell[t]{\textbf{0.760} \\ (0.571, 0.923)} & \makecell[t]{0.600 \\ (0.400, 0.800)} & \makecell[t]{0.526 \\ (0.364, 0.688)} & \makecell[t]{0.526 \\ (0.370, 0.688)} & \makecell[t]{\textbf{0.605} \\ (0.442, 0.756)} \\
 &  & Specificity & \makecell[t]{0.759 \\ (0.726, 0.793)} & \makecell[t]{0.743 \\ (0.709, 0.776)} & \makecell[t]{\textbf{0.802} \\ (0.770, 0.832)} & \makecell[t]{0.691 \\ (0.666, 0.717)} & \makecell[t]{\textbf{0.765} \\ (0.741, 0.787)} & \makecell[t]{0.758 \\ (0.735, 0.781)} \\
 &  & AUROC & \makecell[t]{0.773 \\ (0.682, 0.855)} & \makecell[t]{0.802 \\ (0.743, 0.851)} & \makecell[t]{\textbf{0.807} \\ (0.720, 0.881)} & \makecell[t]{0.716 \\ (0.642, 0.786)} & \makecell[t]{\textbf{0.772} \\ (0.714, 0.829)} & \makecell[t]{0.769 \\ (0.699, 0.831)} \\
\hline
\hline
\multirow[c]{8}{*}{MLP} & \multirow[c]{4}{*}{Voice} & Balanced Accuracy & \makecell[t]{\textbf{0.683} \\ (0.576, 0.784)} & \makecell[t]{0.632 \\ (0.533, 0.727)} & \makecell[t]{0.581 \\ (0.478, 0.688)} & \makecell[t]{\textbf{0.628} \\ (0.547, 0.705)} & \makecell[t]{0.610 \\ (0.529, 0.689)} & \makecell[t]{0.548 \\ (0.477, 0.616)} \\
 &  & Sensitivity & \makecell[t]{0.520 \\ (0.318, 0.714)} & \makecell[t]{\textbf{0.560} \\ (0.360, 0.750)} & \makecell[t]{0.480 \\ (0.280, 0.697)} & \makecell[t]{0.526 \\ (0.368, 0.676)} & \makecell[t]{0.579 \\ (0.417, 0.735)} & \makecell[t]{\textbf{0.763} \\ (0.622, 0.889)} \\
 &  & Specificity & \makecell[t]{\textbf{0.846} \\ (0.817, 0.873)} & \makecell[t]{0.704 \\ (0.668, 0.740)} & \makecell[t]{0.682 \\ (0.646, 0.718)} & \makecell[t]{\textbf{0.729} \\ (0.706, 0.753)} & \makecell[t]{0.640 \\ (0.615, 0.667)} & \makecell[t]{0.333 \\ (0.308, 0.358)} \\
 &  & AUROC & \makecell[t]{\textbf{0.754} \\ (0.643, 0.857)} & \makecell[t]{0.709 \\ (0.637, 0.779)} & \makecell[t]{0.638 \\ (0.514, 0.746)} & \makecell[t]{\textbf{0.692} \\ (0.607, 0.772)} & \makecell[t]{0.633 \\ (0.538, 0.727)} & \makecell[t]{0.575 \\ (0.489, 0.657)} \\
\cline{2-9}
 & \multirow[c]{4}{*}{\makecell[c]{Voice + \\ Demographics}} & Balanced Accuracy & \makecell[t]{0.629 \\ (0.522, 0.730)} & \makecell[t]{\textbf{0.755} \\ (0.659, 0.841)} & \makecell[t]{0.655 \\ (0.556, 0.762)} & \makecell[t]{0.669 \\ (0.586, 0.748)} & \makecell[t]{\textbf{0.696} \\ (0.612, 0.775)} & \makecell[t]{0.657 \\ (0.573, 0.742)} \\
 &  & Sensitivity & \makecell[t]{0.440 \\ (0.227, 0.640)} & \makecell[t]{\textbf{0.760} \\ (0.571, 0.923)} & \makecell[t]{0.440 \\ (0.250, 0.654)} & \makecell[t]{0.553 \\ (0.390, 0.704)} & \makecell[t]{\textbf{0.658} \\ (0.488, 0.813)} & \makecell[t]{0.500 \\ (0.333, 0.667)} \\
 &  & Specificity & \makecell[t]{0.819 \\ (0.786, 0.847)} & \makecell[t]{0.750 \\ (0.717, 0.784)} & \makecell[t]{\textbf{0.871} \\ (0.844, 0.897)} & \makecell[t]{0.786 \\ (0.764, 0.808)} & \makecell[t]{0.734 \\ (0.708, 0.758)} & \makecell[t]{\textbf{0.815} \\ (0.794, 0.835)} \\
 &  & AUROC & \makecell[t]{0.758 \\ (0.663, 0.833)} & \makecell[t]{\textbf{0.809} \\ (0.753, 0.858)} & \makecell[t]{0.805 \\ (0.725, 0.881)} & \makecell[t]{0.715 \\ (0.627, 0.789)} & \makecell[t]{0.758 \\ (0.695, 0.822)} & \makecell[t]{\textbf{0.762} \\ (0.695, 0.826)} \\
\hline
\hline
\multirow[c]{8}{*}{\makecell[c]{Logistic \\Regression}} & \multirow[c]{4}{*}{Voice} & Balanced Accuracy & \makecell[t]{0.653 \\ (0.551, 0.750)} & \makecell[t]{0.663 \\ (0.555, 0.761)} & \makecell[t]{\textbf{0.666} \\ (0.563, 0.767)} & \makecell[t]{\textbf{0.619} \\ (0.541, 0.689)} & \makecell[t]{0.565 \\ (0.487, 0.644)} & \makecell[t]{0.528 \\ (0.438, 0.603)} \\
 &  & Sensitivity & \makecell[t]{0.560 \\ (0.360, 0.762)} & \makecell[t]{\textbf{0.640} \\ (0.429, 0.833)} & \makecell[t]{0.600 \\ (0.400, 0.807)} & \makecell[t]{\textbf{0.711} \\ (0.558, 0.849)} & \makecell[t]{0.579 \\ (0.428, 0.739)} & \makecell[t]{0.526 \\ (0.355, 0.676)} \\
 &  & Specificity & \makecell[t]{\textbf{0.746} \\ (0.713, 0.779)} & \makecell[t]{0.685 \\ (0.649, 0.721)} & \makecell[t]{0.732 \\ (0.698, 0.766)} & \makecell[t]{0.528 \\ (0.502, 0.557)} & \makecell[t]{\textbf{0.551} \\ (0.524, 0.581)} & \makecell[t]{0.530 \\ (0.503, 0.555)} \\
 &  & AUROC & \makecell[t]{\textbf{0.724} \\ (0.604, 0.834)} & \makecell[t]{0.714 \\ (0.637, 0.790)} & \makecell[t]{0.719 \\ (0.612, 0.825)} & \makecell[t]{\textbf{0.665} \\ (0.578, 0.747)} & \makecell[t]{0.603 \\ (0.497, 0.704)} & \makecell[t]{0.545 \\ (0.439, 0.640)} \\
\cline{2-9}
 & \multirow[c]{4}{*}{\makecell[c]{Voice + \\ Demographics}} & Balanced Accuracy & \makecell[t]{0.657 \\ (0.544, 0.756)} & \makecell[t]{\textbf{0.797} \\ (0.722, 0.859)} & \makecell[t]{0.723 \\ (0.623, 0.816)} & \makecell[t]{0.661 \\ (0.586, 0.735)} & \makecell[t]{\textbf{0.747} \\ (0.683, 0.800)} & \makecell[t]{0.701 \\ (0.626, 0.774)} \\
 &  & Sensitivity & \makecell[t]{0.560 \\ (0.345, 0.750)} & \makecell[t]{\textbf{0.880} \\ (0.733, 1.000)} & \makecell[t]{0.680 \\ (0.500, 0.864)} & \makecell[t]{0.711 \\ (0.558, 0.849)} & \makecell[t]{\textbf{0.842} \\ (0.714, 0.947)} & \makecell[t]{0.684 \\ (0.537, 0.829)} \\
 &  & Specificity & \makecell[t]{0.754 \\ (0.722, 0.787)} & \makecell[t]{0.715 \\ (0.677, 0.749)} & \makecell[t]{\textbf{0.767} \\ (0.732, 0.799)} & \makecell[t]{0.612 \\ (0.587, 0.639)} & \makecell[t]{0.652 \\ (0.627, 0.678)} & \makecell[t]{\textbf{0.718} \\ (0.694, 0.743)} \\
 &  & AUROC & \makecell[t]{0.733 \\ (0.627, 0.827)} & \makecell[t]{\textbf{0.836} \\ (0.767, 0.892)} & \makecell[t]{0.813 \\ (0.738, 0.883)} & \makecell[t]{0.687 \\ (0.607, 0.762)} & \makecell[t]{0.777 \\ (0.719, 0.828)} & \makecell[t]{\textbf{0.782} \\ (0.721, 0.838)} \\

\end{tabular}



\caption{Classification results for each of the three acoustic features used alone and when combined with the demographics. These models are evaluated on both a holdout test set from the FEMH dataset and externally on the SVD dataset. Bold values are the highest for that metric and test set. SVM - support vector machine, MLP - multi-layered perceptron.}
\label{tab:ClassificationResults}
% \end{adjustwidth}
\end{table*}

==> title_page.tex <==
\title{Detecting Throat Cancer from Speech Signals using Machine Learning: A Scoping Literature Review}
\author[first]{Mary Paterson}
\affiliation[first]{organization={Faculty of Engineering and Physical Sciences University of Leeds},%Department and Organization 
            city={Leeds},
            country={UK}}
            
\author[second]{James Moor}
\affiliation[second]{organization={Ear, Nose and Throat Department Leeds Teaching Hospitals NHS Trust},%Department and Organization
            city={Leeds},
            country={UK}}

\author[first]{Luisa Cutillo}

Corresponding author is Mary Paterson

email:scmlp@leeds.ac.uk
